FlexFL: Heterogeneous Federated Learning via APoZ-Guided Flexible Pruning in Uncertain Scenarios

Along with the increasing popularity of Deep Learning (DL) techniques, more and more Artificial Intelligence of Things (AIoT) systems are adopting federated learning (FL) to enable privacy-aware collaborative learning among AIoT devices. However, due to the inherent data and device heterogeneity issues, existing FL-based AIoT systems suffer from the model selection problem. Although various heterogeneous FL methods have been investigated to enable collaborative training among heterogeneous models, there is still a lack of i) wise heterogeneous model generation methods for devices, ii) consideration of uncertain factors, and iii) performance guarantee for large models, thus strongly limiting the overall FL performance. To address the above issues, this paper introduces a novel heterogeneous FL framework named FlexFL. By adopting our Average Percentage of Zeros (APoZ)-guided flexible pruning strategy, FlexFL can effectively derive best-fit models for heterogeneous devices to explore their greatest potential. Meanwhile, our proposed adaptive local pruning strategy allows AIoT devices to prune their received models according to their varying resources within uncertain scenarios. Moreover, based on self-knowledge distillation, FlexFL can enhance the inference performance of large models by learning knowledge from small models. Comprehensive experimental results show that, compared to state-of-the-art heterogeneous FL methods, FlexFL can significantly improve the overall inference accuracy by up to 14.24%.

==> comment.tex <==
% !TeX spellcheck = en_US
\clearpage
\setcounter{section}{0}
\section{Responses to Reviewer Comments}
%\newcounter{cntcmmt}[subsection]
\newcounter{cntcmmt}

%\footnotesize
\newcommand{\Reviewer}
{\subsection{REVIEWER \arabic{subsection}}}

\newcommand{\Cmnt}[1]
{ 
\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\noindent {\bf Comment \stepcounter{cntcmmt}\arabic{cntcmmt}:}
{\it #1} \vspace{0.0in}
\end{tcolorbox}
}

\newcommand{\Rsp}[1]
{{\bf Response:} #1 \vspace{0.020in}}


\def\commref#1{Comment~\ref{#1}}

% \def\tableoverhead{
% \begin{table}[!h]
% \centering
% \vspace{-0.15in}
% \caption{Comparison of training time, dispatch, and upload overhead to achieve target inference accuracy (VGG on IID CIFAR10).}
% \label{Table comment: overhead}
% \vspace{-0.1in}
% \scriptsize
% \begin{tabular}{cc|cccc}
% \hline
% \multicolumn{2}{c|}{Target Accuracy}                                                                     & 70\%    & 75\%    & 80\%     & 85\%     \\ \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{FlexFL}}                                                            & Time (s)      & 4849  & 6857  & 11736  & 32810  \\
% \multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 18337 & 26580 & 45860  & 132298 \\
% \multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 17751 & 25914 & 44736  & 129075 \\ \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{FlexFL\\ w/o self-KD}}} & Time (s)      & 2566  & 4013  & 7985   & N/A      \\
% \multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 16520 & 28767 & 59857  & N/A      \\
% \multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 16022 & 27973 & 58208  & N/A      \\ \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{ScaleFL}}                                                           & Time (s)      & 9566  & 14808 & 77926  & N/A      \\
% \multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 35935 & 55727 & 300499 & N/A      \\
% \multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 34252 & 53226 & 288020 & N/A      \\ \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{HeteroFL}}                                                          & Time (s)      & 4900  & 8328  & N/A      & N/A     \\
% \multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 26412 & 45624 & N/A      & N/A      \\
% \multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 24023 & 41822 & N/A      & N/A      \\ \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{All Large}}                                                          & Time (s)     & 3821  & N/A     & N/A      & N/A      \\
% \multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 37684 & N/A     & N/A      & N/A      \\
% \multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 37684 & N/A     & N/A      & N/A      \\ \hline
% \end{tabular}
% \end{table}
% }

% \def\tablegamma{
% \begin{table}[!h]
% \centering
% \vspace{-0.15in}
% \caption{Accuracy comparison with different adaptive pruning sizes (VGG ON IID CIFAR10).}
% \vspace{-0.1in}
% \label{Table comment: adaptive size}
% \scriptsize
% \begin{tabular}{ccc}
% \hline
% Adaptive Pruning Size $\Gamma$ & Global Model Acc & Avg Model Acc \\ \hline
% 1\%                         & 84.38\%             & 84.22\%           \\
% 2\%                        & 84.86\%            & 84.65\%          \\
% 5\%                        & 84.88\%            & 84.67\%          \\
% 10\%                          & 85.16\%               & 84.75\%             \\
% 15\%                        & 84.40\%              & 84.21\%            \\ \hline
% \end{tabular}
% \vspace{-0.1in}
% \end{table}
% }
% %\textcolor[rgb]{1,0,0}{{\bf Note that 
% %the original log number of this manuscript is TC-2019-01-0001.R2}}.

We would like to thank the reviewers for their insightful comments. 
 We have revised the manuscript to address various issues raised by the reviewers. 
This section summarizes all the reviewer
 comments and our responses in terms of how we have addressed the
 issues in the revised manuscript. 


% \def\tableablation{
% \begin{table}[!h]
% \centering
% \vspace{-0.15in}
% \caption{FlexFL distillation and adaptive pruning overhead ablation (VGG ON IID CIFAR10).}
% \label{Table comment: FlexFL distillation and adaptive pruning overhead ablation}
% \scriptsize
% \vspace{-0.15in}

% \begin{tabular}{c|c|ccc}
% \hline
% Method                                                                            & Dispatch & Ada. Pruning  & Local Train      & Total   \\ \hline
% \multirow{4}{*}{FlexFL}                                                           & 100\%          & 1.45s (1.3\%)  & 108.59s (98.7\%) & 110.04s \\
%                                                                                   & 50\%           & 1.45s (1.9\%)  & 73.92s (98.1\%)  & 75.37s  \\
%                                                                                   & 25\%           & 0s (0\%)       & 46.06s (100\%)   & 46.06s  \\ \cline{2-5} 
%                                                                                   & Avg       & 1.45s (2.0\%) & 70.37s (98.0\%)  & 71.82s  \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}FlexFL  \\ w/o self-KD\end{tabular}} & 100\%          & 1.44s (2.2\%) & 64.17s (97.8\%)  & 65.61s  \\
%                                                                                   & 50\%           & 1.45s (2.6\%) & 52.88s (97.4\%)  & 54.33s  \\
%                                                                                   & 25\%           & 0s (0\%)             & 45.77s (100\%)   & 45.77s  \\ \cline{2-5} 
%                                                                                   & Avg        & 1.44s (2.8\%) & 50.61s (97.2\%)  & 52.05s  \\ \hline
% \end{tabular}
% \end{table}

% }



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %review1
\Reviewer

\Cmnt{Accuracy has detailed evaluation and similar needs to be considered for performance or speedup.}


\Rsp{Thanks for the suggestion.
To evaluate the performance and speedup our approach achieved, we conducted new experiments on FlexFL and the three baselines with specified 
target accuracy (i.e., 70\%, 75\%, 80\%, and 85\%). 
The following Table~\ref{Table comment: overhead} shows the experimental
results. Note that we use the notation ``N/A'' to denote that a specified algorithm cannot achieve its target accuracy. 

\begin{table}[!h]
\centering
\vspace{-0.05in}
\caption{Comparison of Training Time for Different Target Accuracy (VGG on IID CIFAR10).}
\label{Table comment: overhead}
%\vspace{-0.1in}
\scriptsize
\begin{tabular}{cc|cccc}
\hline
\multicolumn{2}{c|}{Target Accuracy}                                                                     & 70\%    & 75\%    & 80\%     & 85\%     \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{FlexFL}}                                                            & Time (s)      & 4849  & 6857  & 11736  & 32810  \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 18337 & 26580 & 45860  & 132298 \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 17751 & 25914 & 44736  & 129075 \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{FlexFL\\ w/o self-KD}}} & Time (s)      & 2566  & 4013  & 7985   & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 16520 & 28767 & 59857  & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 16022 & 27973 & 58208  & N/A      \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{ScaleFL}}                                                           & Time (s)      & 9566  & 14808 & 77926  & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 35935 & 55727 & 300499 & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 34252 & 53226 & 288020 & N/A      \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{HeteroFL}}                                                          & Time (s)      & 4900  & 8328  & N/A      & N/A     \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 26412 & 45624 & N/A      & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 24023 & 41822 & N/A      & N/A      \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{All Large}}                                                          & Time (s)     & 3821  & N/A     & N/A      & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 37684 & N/A     & N/A      & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 37684 & N/A     & N/A      & N/A      \\ \hline
\end{tabular}
\end{table}

From this table, we can find that FlexFL converges to target accuracy much faster than all the baselines except ``All Large''. Moreover, FlexFL can achieve an accuracy of 85\%, while all the other methods fail.  
Specifically, compared with ScaleFL, FlexFL can achieve a training speedup of up to 6.63$\times$ and a reduction of communication overhead (Dispatch+Upload) by up to 85\%. 
% As shown in , compared to ScaleFL and HeteroFL, FlexFL can achieve the target accuracy with the least communication and time overhead in all the cases.
% Specifically, our FlexFL can achieve a 1.97$\times$-6.63$\times$ speedup and 49\%-85\% reduction in upload and dispatch communication overhead compared to ScaleFL.
% Compared with HeteroFL, our FlexFL can achieve a 1.01$\times$-1.21$\times$ speedup and 31\%-42\% reduction.
% Although the baseline ``All Large'' can achieve 70\% accuracy more fast than FlexFL, but it costs about 1.05$\times$ more communication overhead than FlexFL. In addition, the baseline ``All Large'' cannot achieve higher accuracy. FlexFL without self-KD can achieve the same accuracy faster than FlexFL but may suffer more communication overhead.
%
We have revised the paper and included the above experimental results in 
Section~\ref{sec : Training Time and Communication Overhead Analysis} (see page 11).


% We added the comparison of the overhead between our method and 3 baselines, with detailed content in section \ref{sec : Training Time and Communication Overhead Analysis}. We use the time to reach the same accuracy as the standard. As shown in table \ref{Table: overhead}, our method reaches the same accuracy faster 1.97$\times$-6.63$\times$ compared to ScaleFL and requires 49\%-85\% less upload and dispatch communication overhead than ScaleFL.
}




%%%%%done
\Cmnt{Heterogeneous Model Generation step needs more details on what/how exactly it has been done.}


% % list point
% \Rsp{Sorry for the confusion. The Heterogeneous Model Generation step primarily involves calculating the pruning ratio for the model based on the APoZ values and adjusted APoZ values, and then generating models corresponding to these ratios. 
% The APoZ values and adjusted APoZ values can be obtained from the formulas in equation \ref{eq: APoZ},\ref{eq: blockAPOZ},\ref{eq: AdjW}. The specific method for generating pruning ratios can be found in lines \ref{Al2:while_start}-\ref{Al2:12} of Algorithm \ref{algorithm: Generate}, resulting in a vector of length $ \text{len}(M) $, where each element represents the pruning ratio for the corresponding layer. The pruning ratios are derived from the formula $\mathbb{R}^{(y_j \times s[i][j]) \times (x_j \times s[i][j-1])}$ to obtain the pruned model. For example, assume that the first convolutional layer of model $ M_i $ has 3 input and 64 output channels. If $ s[i][0] $ is 0.5, then the filter number of the first layer will be pruned to $ 64 \times 0.5 = 32 $, and the number of input channels in the second convolutional layer will also be adjusted to 32.  We have revised Section \ref{sec: Model Gen} to add the above expressions.
% }
\Rsp{
Sorry for the confusion. 
Our heterogeneous model generation step involves three main steps: 
i) calculating the  APoZ scores $A_j$  and adjustment weights $AdjW_j$ for $j^{th}$ layer;
%
ii) finding an appropriate $s[i][j]$ for each layer $j$ in model $M_i$, so that the size of a model $M_i$ matches its target size $L_p[i]$; 
%
and iii) generating models $M_i$ according to the obtained $s[i][]$.
%
The details of these three steps are as follows:
%
\begin{itemize}
    \item \textbf{Step 1:} We calculate the APoZ score $A_j$ and  adjustment weight $AdjW_j$ according to
    Equations~\ref{eq: APoZ}-~\ref{eq: AdjW}.
    \item \textbf{Step 2:} We calculate  $s[i][j]$ ($j\leq \text{len}(M)$) based    
    on the Lines~\ref{Al2:while_start}-~\ref{Al2:prune_end} of Algorithm~\ref{algorithm: Generate}, where  $s[i][j]$ indicates the pruning ratio for the $j^{th}$ layer of model $M_i$.
    % The specific method for generating pruning ratios $s[i][j]$ can be found in Lines~\ref{Al2:while_start}-~\ref{Al2:12} of Algorithm~\ref{algorithm: Generate}, resulting in a vector of length $ \text{len}(M) $, where each element represents the pruning ratio for the corresponding layer.
    %
%    
    \item \textbf{Step 3:} Let $ x_{j} $ and  $ y_{j} $ be the numbers of input channels and output channels of the $j^{th}$ layer of model $M$, respectively. 
   For  $j$ ($1\leq j\leq len(M)$), we prune the $j^{th}$ layer of model $M$   based on $ s[i][j] $ obtained in step 2, and get a new  model  $M_i$ with $x_j\times s[i][j-1]$ input channels and $y_i \times s[i][j]$  output channels. The pruned model is then added to the model pool $P$. 
    %
    For example, assume that the second convolutional layer of model $M$ has 64 input and 128 output channels.
    %
    If $ s[i][1] $ is 0.25 and $ s[i][2] $ is 0.5, after the pruning, 
    the numbers of input and output channels of the second layer will be $64 \times 0.25 = 16$   and   $128 \times 0.5 = 64$, respectively.
\end{itemize}
%
We have revised the paper in Section~\ref{sec: Model Gen} (see pages 4-5).
% 1) The APoZ values and adjusted APoZ values can be obtained from the formulas in equation~\ref{eq: APoZ},\ref{eq: blockAPOZ},\ref{eq: AdjW}. We calculate the pruning ratio $s[i][j]$ based on these values. 
% 2) The specific method for generating pruning ratios $s[i][j]$ can be found in lines~\ref{Al2:while_start}-~\ref{Al2:12} of Algorithm~\ref{algorithm: Generate}, resulting in a vector of length $ \text{len}(M) $, where each element represents the pruning ratio for the corresponding layer.
% 3) The pruning ratios are derived from the formula $\mathbb{R}^{(y_j \times s[i][j]) \times (x_j \times s[i][j-1])}$ to obtain the pruned model. For example, assume that the first convolutional layer of model $ M_i $ has 3 input and 64 output channels. If $ s[i][0] $ is 0.5, then the filter number of the first layer will be pruned to $ 64 \times 0.5 = 32 $, and the number of input channels in the second convolutional layer will also be adjusted to 32.  
% We have added the examples above to express the generation step better in Section~\ref{sec: Model Gen}.
}

% model device point
\Cmnt{What exact resource configurations are considered in the model and device selection?}

\Rsp{
% r = 1代表1%的模型参数大小
In this paper, we focus on the memory usage of devices.
 Table~\ref{Table: Resource distribution table} presents the memory configurations (i.e., $r$) for device selection.  For example, if $r$ is 30, the number of parameters of a pruned model cannot exceed   30\%  of its original counterpart. 
 We have revised the paper and included the above description in 
 Section~\ref{sec: device settings} (see pages 6-7).
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\Cmnt{In Adaptive Local Pruning, how to determine that available resources are insufficient to train the achieved model? 
}

\Rsp{
As mentioned in Section~\ref{subsubsec: Device Heterogeneity Settings}, if 
the device memory is smaller than a dispatched model $m$, i.e., $r \leq \frac{\text{size}(m)}{\text{size}(M)}\times 100$, our approach will not train $m$ due to insufficient memory resources. 
In this case,  $m$ will be pruned to be an adaptive model to fit the device (see pages 6-7). 
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Cmnt{How the 10\% pruning is determined. This is the most important contribution and needs elaboration.}

\Rsp{Sorry for the confusion. We conducted experiments to evaluate the impact of adaptive pruning sizes $\Gamma$. 

\begin{table}[!h]
\centering
\vspace{-0.05in}
\caption{Test accuracy comparison with different $\Gamma$.}
%\vspace{-0.1in}
\label{Table comment: adaptive size}
\scriptsize
\begin{tabular}{ccc}
\hline
 $\Gamma$ & Global  Accuracy & Avg  Accuracy \\ \hline
1\%                         & 84.38\%             & 84.22\%           \\
2\%                        & 84.86\%            & 84.65\%          \\
5\%                        & 84.88\%            & 84.67\%          \\
10\%                          & 85.16\%               & 84.75\%             \\
15\%                        & 84.40\%              & 84.21\%            \\ \hline
\end{tabular}
%\vspace{-0.1in}
\end{table}

From the above table, we can find that $\Gamma = 10\%$ is the best choice in an empirical manner. 
% It is notable that if the adaptive pruning size is too small, it leads to lower utilization of buffered models in the same uncertainty scenario, meaning more devices will directly degrade to the next-level model.
% Conversely, if the adaptive pruning size is too large, although the utilization of buffered models improves, the utilization of devices becomes insufficient, resulting in nearly the same performance between pruning to buffered models and direct degradation to the next-level model. 
We have modified the paper and included the explanation in  Section~\ref{sec: Adaptive Local Model Pruning Size} (see page 9).
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\Cmnt{It is also not clear how adaptation will work under uncertain scenarios as claimed earlier or when variation in device availability happens. Consideration of such variations has been done in different contexts like in `Collaborative Adaptation for Energy-Efficient Heterogeneous Mobile SoCs', and those ideas can be refined.}

\Rsp{Sorry for the confusion. 
%
Our approach checks devices' memory usage when they start receiving models dispatched by the cloud server. If a device cannot accommodate its specified model, it will locally conduct adaptive pruning. 

We agree that there are many works (e.g., \cite{singh2019collaborative}) that deal with resource variations adaptively. 
We have added more references and corresponding descriptions to enrich the background of our approach (see page 1).  

%{\color{red} TODO}

% Our method indeed lacks consideration for device factors other than memory, such as CPU usage and current battery level. The adaptive pruning part of our method only proposes a solution to the uncertainty of memory resources. In future work, FlexFL will include other uncertainties on the device and propose corresponding solutions for these factors.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\Cmnt{Overhead evaluation of FlexFL approach as it might do many adaptions in changing scenarios.}



\Rsp{
We conducted new experiments to evaluate the overhead introduced by each component of our method. The experimental results are as follows. 
%
\begin{table}[!h]
\centering
\vspace{-0.05in}
\caption{Ablation results of  distillation overhead and adaptive pruning overhead for FlexFL
 (VGG on IID CIFAR10).}
\label{Table comment: FlexFL distillation and adaptive pruning overhead ablation}
\scriptsize
\vspace{-0.1in}
\begin{tabular}{c|c|ccc}
\hline
\multirow{2}{*}{Method}                                                                            & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dispatched  \\ Model Size\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Adaptive  \\ Pruning \end{tabular}}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Local  \\ Training\end{tabular}}      & \multirow{2}{*}{Total}  \\
& & & & \\ \hline
\multirow{4}{*}{FlexFL}                                                           & 100\%          & 1.45s (1.3\%)  & 108.59s (98.7\%) & 110.04s \\
                                                                                  & 50\%           & 1.45s (1.9\%)  & 73.92s (98.1\%)  & 75.37s  \\
                                                                                  & 25\%           & 0s (0\%)       & 46.06s (100\%)   & 46.06s  \\ \cline{2-5} 
                                                                                  & Avg       & 1.45s (2.0\%) & 70.37s (98.0\%)  & 71.82s  \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}FlexFL  \\ w/o self-KD\end{tabular}} & 100\%          & 1.44s (2.2\%) & 64.17s (97.8\%)  & 65.61s  \\
                                                                                  & 50\%           & 1.45s (2.6\%) & 52.88s (97.4\%)  & 54.33s  \\
                                                                                  & 25\%           & 0s (0\%)             & 45.77s (100\%)   & 45.77s  \\ \cline{2-5} 
                                                                                  & Avg        & 1.44s (2.8\%) & 50.61s (97.2\%)  & 52.05s  \\ \hline
\end{tabular}
%\vspace{-0.1in}
\end{table}

From this table, we can find that ``FlexFL w/o self-KD'' needs 52.05s on average, while FlexFL needs 71.82s on average. Obviously, the introduction of self-KD will result in longer local training time. 
Note that our method's pre-processing time accounts for approximately 0.3\% of the total training time (for 1000 rounds of training), and its adaptive pruning time accounts for about 3\% of the local time. 
Compared with the overall training time, such costs are negligible. 
We have revised the paper and added the above explanation in 
Section~\ref{sec: overhead ablation} (see page 11).
}







\Cmnt{Grammar issues, e.g.:about model heterogeneous FL, the could server aggregates.}

\Rsp{Thanks for pointing out the grammar errors. 
We have scanned the paper carefully and corrected all of them.
}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \Cmnt{about model heterogeneous FL}

% \Rsp{

% }
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \Cmnt{the could server aggregates}

% \Rsp{

% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%review2
%%%%%%%%%%%%%%%%%%%%%%%%%%


\Reviewer

%%%%%done
\Cmnt{The additional overheads for each of APoZ-guided pruning, adaptive local pruning, self-knowledge distillation should be evaluated in terms of computation cost and working memory size, in order to demonstrate that these techniques can decrease the computation costs compared to simply training the large models.}

% \Rsp{Sorry for the confusion. We have conducted new experiments  to evaluate the additional overhead introduced by each component of our method.
% As shown in Table \ref{Table: FlexFL distillation and adaptive pruning overhead ablation}, introducing self-KD increases the time overhead by 1.37$\times$ but does not add any extra communication overhead. 
% The pre-processing time of our method accounts for approximately 0.3\% of the total training time (for 1000 rounds of training), and the adaptive pruning time of our method accounts for about 3\% of the local time.
% In terms of memory usage, APoZ-guided pruning is performed on the server side, which prevents memory bottlenecks. 
% Adaptive local pruning prunes the model to a smaller or equivalent size based on resource constraints, and since the model becomes smaller, it will not result in increased memory consumption.
% Self-knowledge distillation will distill a model smaller than the original, so the device's memory still be able to afford the model when loading it.
% In heterogeneous federated learning scenarios, training with a large model on all devices is impractical due to the excessive memory consumption, making it impossible to train the large model on medium or weak devices. In section \ref{sec : Training Time and Communication Overhead Analysis}, we compared FlexFL with three other baselines. Among them, AllLarge represents the results obtained by training only on strong clients. We found that, compared to the other baselines, our method performs better in terms of time and communication overhead.

% }
\Rsp{Thanks for your suggestion. 
%
We conducted new experiments to evaluate the additional overhead introduced by each component of our method. The results are as follows.
\begin{table}[!h]
\centering
\vspace{-0.05in}
\caption{Ablation results of  distillation overhead and adaptive pruning overhead for FlexFL
 (VGG on IID CIFAR10).}
\label{ablation_1}
\scriptsize
%\vspace{-0.1in}
\begin{tabular}{c|c|ccc}
\hline
\multirow{2}{*}{Method}                                                                            & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dispatched  \\ Model Size\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Adaptive  \\ Pruning \end{tabular}}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Local  \\ Training\end{tabular}}      & \multirow{2}{*}{Total}  \\
& & & & \\ \hline
\multirow{4}{*}{FlexFL}                                                           & 100\%          & 1.45s (1.3\%)  & 108.59s (98.7\%) & 110.04s \\
                                                                                  & 50\%           & 1.45s (1.9\%)  & 73.92s (98.1\%)  & 75.37s  \\
                                                                                  & 25\%           & 0s (0\%)       & 46.06s (100\%)   & 46.06s  \\ \cline{2-5} 
                                                                                  & Avg       & 1.45s (2.0\%) & 70.37s (98.0\%)  & 71.82s  \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}FlexFL  \\ w/o self-KD\end{tabular}} & 100\%          & 1.44s (2.2\%) & 64.17s (97.8\%)  & 65.61s  \\
                                                                                  & 50\%           & 1.45s (2.6\%) & 52.88s (97.4\%)  & 54.33s  \\
                                                                                  & 25\%           & 0s (0\%)             & 45.77s (100\%)   & 45.77s  \\ \cline{2-5} 
                                                                                  & Avg        & 1.44s (2.8\%) & 50.61s (97.2\%)  & 52.05s  \\ \hline
\end{tabular}
\vspace{-0.15in}
\end{table}


{\bf Additional Computation Cost.} From Table~\ref{ablation_1}, we can find that  FlexFL without self-KD needs 52.05s on average, while FlexFL needs 71.82s on average. Obviously, the introduction of self-KD will result in longer local training time. 
Note that our method's pre-processing time accounts for approximately 0.3\% of the total training time (for 1000 rounds of training), and its adaptive pruning time accounts for about 3\% of the local time. Compared with the overall training time, such costs are negligible. 

{\bf Additional Working Memory Size.}  Since APoZ-guided pruning, adaptive local pruning, and self-distillation do not 
rely on any complex data structures, the additional memory overhead they introduce is negligible.
Note that APoZ-guided pruning is performed on the server side and only once upon initialization, it does not impose any burden on devices. 


\begin{table}[!h]
\centering
\vspace{-0.15in}
\caption{Comparison of Training Time for Different Target Accuracy.}
\label{Table comment: overhead1}
\vspace{-0.1in}
\scriptsize
\begin{tabular}{cc|cccc}
\hline
\multicolumn{2}{c|}{Target Accuracy}                                                                     & 70\%    & 75\%    & 80\%     & 85\%     \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{FlexFL}}                                                            & Time (s)      & 4849  & 6857  & 11736  & 32810  \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 18337 & 26580 & 45860  & 132298 \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 17751 & 25914 & 44736  & 129075 \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{FlexFL\\ w/o self-KD}}} & Time (s)      & 2566  & 4013  & 7985   & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 16520 & 28767 & 59857  & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 16022 & 27973 & 58208  & N/A      \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{ScaleFL}}                                                           & Time (s)      & 9566  & 14808 & 77926  & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 35935 & 55727 & 300499 & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 34252 & 53226 & 288020 & N/A      \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{HeteroFL}}                                                          & Time (s)      & 4900  & 8328  & N/A      & N/A     \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 26412 & 45624 & N/A      & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 24023 & 41822 & N/A      & N/A      \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{All Large}}                                                          & Time (s)     & 3821  & N/A     & N/A      & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Dispatch (MB) & 37684 & N/A     & N/A      & N/A      \\
\multicolumn{1}{c|}{}                                                                                   & Upload (MB)   & 37684 & N/A     & N/A      & N/A      \\ \hline
\end{tabular}
\vspace{-0.1in}
\end{table}

We also conducted new experiments to show that these techniques can decrease the computation costs compared to ``All Large'' method that simply trains large models. Table~\ref{Table comment: overhead1} shows the experimental results. 
We can find that although FlexFL is slightly slower than ``All Large'', it can achieve all the accuracy targets, while ``All Large'' can only achieve an accuracy of up to 70\%. 
Note that we also tried FlexFL without self-distillation, we can find our approach is faster than  ``All Large'', and can achieve an accuracy of up to 80\%.
We have revised the paper and included the above discussion in Section~\ref{sec : Training Time and Communication Overhead Analysis} and Section~\ref{sec: overhead ablation} (see page 11).
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%review3
\Reviewer


\Cmnt{Why consider pruning 10\% in the first place? Is there a better pruning ratio? }

\Rsp{
Sorry for the confusion. We conducted experiments to evaluate the impact of adaptive pruning sizes $\Gamma$. 

\begin{table}[!h]
\centering
\vspace{-0.15in}
\caption{Test accuracy comparison with different $\Gamma$.}
\vspace{-0.1in}
\label{Table comment: adaptive size}
\scriptsize
\begin{tabular}{ccc}
\hline
 $\Gamma$ & Global  Accuracy & Avg  Accuracy \\ \hline
1\%                         & 84.38\%             & 84.22\%           \\
2\%                        & 84.86\%            & 84.65\%          \\
5\%                        & 84.88\%            & 84.67\%          \\
10\%                          & 85.16\%               & 84.75\%             \\
15\%                        & 84.40\%              & 84.21\%            \\ \hline
\end{tabular}
\vspace{-0.1in}
\end{table}

From the above table, we can find that $\Gamma = 10\%$ is the best choice in an empirical manner. 
We have modified the paper and included the explanation in  Section~\ref{sec: Adaptive Local Model Pruning Size} (see page 9).
}
% When a device's resources are insufficient to afford the adaptive pruning model, it downgrades to the next-level model. For example, if the dispatched model is $M_3$ and the resources are insufficient, it will be adaptively pruned to $M^\prime_3$. If the device cannot afford the adaptive pruned model, it will downgrade to $M_2$, then check the device's resource status and repeat the process until the device's resources are sufficient.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Cmnt{...whether the local pruning method in the device is the same as the pruning on the cloud server? If so, how to choose the granularity of the lower-level model in local pruning?}

\Rsp{
Sorry for the confusion. Both the cloud server and clients adopt the same pruning strategy. 
%
Generally,  a FlexFL user is allowed to specify its own granularity to perform local pruning.
%
By default, FlexFL uses three pruning ratios, i.e., 100\% for $M_3$, 50\% for $M_2$, and 25\% for $M_1$ with two adaptive pruning ratios, i.e., $100\%-\Gamma$ for $M^\prime_3$, and $50\%-\Gamma$ for $M^\prime_2$, where $\Gamma$ is a constant hyperparameter. 
%
For example, if a model of type $M_3$ is dispatched to some device with insufficient resources, the client will adaptively prune the model in the order of  $M^\prime_3$, $M_2$,  $M^\prime_2$, and $M_1$ until the pruned model can be accommodated by the device (see page 5). 
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Cmnt{It needs to further distinguish the contribution boundaries. 
For instance, both the APoZ-based pruning strategy and local training utilizing self-knowledge distillation are commonly employed techniques. 
What sets apart the methods utilized in this study?}
% 全文思想
%%改

% The traditional apoz pruning method uses network pruning and retraining strategy to guide model pruning in a centralized scenario, but the huge overhead of this method and the demand for a centralized dataset are unacceptable in a federated learning scenario. Specifically, our method has the following differences: 1) we only need to obtain APoZ once to guide the pruning without re-training, which reduces the computational overhead; 2). Propose to adjust the weight; 3)Only 1\ of the protocol dataset is needed, no centralized full dataset is needed

\Rsp{Sorry for the confusion. 
Our approach is significantly different from existing methods, especially  APoZ-based pruning methods, and self-KD-based FL methods, since:
{\bf First}, the goals of existing APoZ-based methods and FlexFL are different. 
     Although both are based on pruning, the former focuses on model pruning to fit a target device, while the latter aims to enable knowledge sharing among heterogeneous devices. Note that our approach uses adjustment weights to maximize the knowledge-sharing performance.
   {\bf Second}, the purposes of self-KD in FlexFL and existing self-KD-based FL methods are different. 
     Specifically, existing  FL methods adopt self-KD to facilitate knowledge transfer from large models to small models. Unlike these methods, FlexFL strives to share knowledge from small models to large models. This is because, in heterogeneous FL scenarios, large models cannot be deployed on devices with insufficient resources and are thus less knowledgeable than small models.  
To the best of our knowledge, our work is the first attempt to use APoZ-based pruning to improve the learning performance of heterogeneous FL systems. {\bf We have revised the whole introduction section (see pages 1-2) and part of the approach section (see pages 3-6) to make the contribution boundaries clearer.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% Our method proposes a heterogeneous federated learning framework aimed at addressing the challenges of heterogeneous federated learning in uncertain scenarios. The APoZ-based pruning method and self-distillation technique are utilized to implement our framework, and we have also made improvements to these methods specifically for heterogeneous federated learning scenarios.

% In the APoZ-based pruning strategy, we use additional APoZ adjustment values to modify the APoZ scores. Based on the findings in papar [{\color{blue} C1}], we discovered that pruning deeper layers first in deep neural networks can minimize the impact on overall network performance and significantly reduce the number of parameters. Therefore, in Section~\ref{sec: APoZ-Guided Model Generation} we use equation \ref{eq: AdjW} to adjust the APoZ values.

% Traditionally, in self-knowledge distillation, small models learn from large models because large models generally have more parameters and higher accuracy. 
% However, due to the characteristics of heterogeneous federated learning, the data on weak devices can only be trained by small models, resulting in higher accuracy for the small models. 
% In Section~\ref{sec: Self-Knowledge Distillation-based Local Training} we adopted a new self-distillation strategy where, during training, the larger model learns from the smaller model.
 % {\color{blue}
 % \small
 % \noindent[C1] H. Li et al., ``Pruning filters for efficient convnets,''  ICLR, 2016.
 % }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Cmnt{This study conducted extensive experimental verification to support the effectiveness of the proposed method. However, there are currently a large number of methods focusing on heterogeneous FL, and it is unclear whether the compared methods are SOTA.}

\Rsp{Sorry for the confusion. 
In the experiment section, we compared FlexFL with three FL methods: FedAvg, Decoupled, HeteroFL, and ScaleFL. FedAvg and Decoupled are the most classic FL methods, and HeteroFL is the first attempt at heterogeneous FL that adopts heterogeneous aggregation. Note that  ScaleFL (published in CVPR 2023) is a SOTA heterogeneous FL method. 




% Decoupled is based on the basic non-aggregated heterogeneous federated learning framework FedAvg. HeteroFL is the first paper in the heterogeneous federated learning field to introduce heterogeneous aggregation. ScaleFL, proposed in 2023, is, to our best knowledge, the latest state-of-the-art in the heterogeneous federated learning domain. Therefore, we chose these three baselines for comparison.
}

% {\color{blue}
% \noindent[1] B. McMahan, E. Moore, D. Ramage, S. Hampson, and B. A. y Arcas, “Communication-efficient learning of deep networks from decentralized data,” in Artificial intelligence and statistics. PMLR, 2017, pp. 1273–1282.\\
% \noindent[2] E. Diao, J. Ding, and V. Tarokh, “Heterofl: Computation and communication efficient federated learning for heterogeneous clients,” 2021.\\
% \noindent[3] F. Ilhan, G. Su, and L. Liu, “Scalefl: Resource-adaptive federated learning with heterogeneous clients,” in Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition, 2023, pp. 24 532–24 541.\\
% }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%review4
\Reviewer

%%%% done
\Cmnt{FlexFL incorporates multiple hyperparameters, such as pruning thresholds and distillation coefficients, which require careful tuning. Finding the optimal settings can be time-consuming and may demand domain-specific expertise.}

%% 2个表一个图？
\Rsp{
Indeed, our approach involves three new hyperparameters. However, we have studied their impacts on FL training performance as shown in Table \ref{Table: similarity}, Table \ref{Table: adaptive size} and Figure  \ref{fig:  Distillation experiment} and found that FlexFL is insensitive to these hyperparameters. 
Therefore, exploring optimal settings for such hyperparameters does not require much time with domain-specific expertise (see pages 8-9).
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\Cmnt{The adoption of complex pruning and distillation mechanisms in FlexFL may exacerbate communication bottlenecks, especially in scenarios with limited bandwidth or high latency.
}



\Rsp{
Sorry for the confusion. 
Since the pruning and self-KD are conducted locally on devices, they will not cause any extra communication overhead (see page 5). 
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\Cmnt{
While FlexFL demonstrates robustness across varying resource distributions, it may be sensitive to the degree of data heterogeneity among devices. In cases where devices have vastly different data distributions or qualities, the performance of FlexFL may degrade due to suboptimal model pruning or distillation.
}

\Rsp{
Sorry for the confusion. 
The goal of our APoZ-based pruning is to maximize knowledge sharing among heterogeneous devices with varying memory sizes, no matter within IID or non-IID scenarios.
Similar to other FL methods, FlexFL can achieve better training performance in IID scenarios than in non-IID scenarios. 
However, from Table \ref{Table: Experiment}, Table \ref{Table: Resource distribution experiment}, and Table \ref{Table: real-world dataset}, we can find that our approach outperforms all the other baselines in both IID and non-IID scenarios (see page 8 and page 10). 
}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Cmnt{The intricate design of FlexFL, coupled with its computational demands and sensitivity to hyperparameters, may limit its scalability to large-scale FL deployments. Implementation challenges may arise when scaling FlexFL to accommodate many heterogeneous devices or complex neural network architectures.
}

\Rsp{
Sorry for the confusion. As shown in  Table \ref{Table: similarity}, Table \ref{Table: adaptive size} and Figure  \ref{fig:  Distillation experiment}, FlexFL is not sensitive to the hyperparameters. 
Moreover, we conducted experiments to evaluate the scalability of FlexFL in Sections \ref{sec: Participating}, \ref{sec: Simultaneously}, and \ref{sec: Proportions}. The experimental results show that our approach can accommodate large FL applications with various network architectures (see pages 8-9).
}



